Interface Theories for (A)synchronously Communicating Modal I/O-Transition Systems

Interface specifications play an important role in component-based software development. An interface theory is a formal framework supporting composition, refinement and compatibility of interface specifications. We present different interface theories which use modal I/O-transition systems as their underlying domain for interface specifications: synchronous interface theories, which employ a synchronous communication schema, as well as a novel interface theory for asynchronous communication where components communicate via FIFO-buffers.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Beno\^it Caillaud and Axel Legay (Eds.):\\
Foundations of Interface Technologies (FIT'10)\\
EPTCS 46, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.46.1}{10.4204/EPTCS.46.1}}
\pdfoutput=1

